Unsupervised Deep Metric Learning with Transformed Attention Consistency and Contrastive Clustering Loss

Existing approaches for unsupervised metric learning focus on exploring self-supervision information within the input image itself. We observe that, when analyzing images, human eyes often compare images against each other instead of examining images individually. In addition, they often pay attention to certain keypoints, image regions, or objects which are discriminative between image classes but highly consistent within classes. Even if the image is being transformed, the attention pattern will be consistent. Motivated by this observation, we develop a new approach to unsupervised deep metric learning where the network is learned based on self-supervision information across images instead of within one single image. To characterize the consistent pattern of human attention during image comparisons, we introduce the idea of transformed attention consistency. It assumes that visually similar images, even undergoing different image transforms, should share the same consistent visual attention map. This consistency leads to a pairwise self-supervision loss, allowing us to learn a Siamese deep neural network to encode and compare images against their transformed or matched pairs. To further enhance the inter-class discriminative power of the feature generated by this network, we adapt the concept of triplet loss from supervised metric learning to our unsupervised case and introduce the contrastive clustering loss. Our extensive experimental results on benchmark datasets demonstrate that our proposed method outperforms current state-of-the-art methods for unsupervised metric learning by a large margin.

==> egbib.tex <==
@article{dosovitskiy2015discriminative,
  title={Discriminative unsupervised feature learning with exemplar convolutional neural networks},
  author={Dosovitskiy, Alexey and Fischer, Philipp and Springenberg, Jost Tobias and Riedmiller, Martin and Brox, Thomas},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={38},
  number={9},
  pages={1734--1747},
  year={2015},
  publisher={IEEE}
}

@inproceedings{wu2018unsupervised,
  title={Unsupervised feature learning via non-parametric instance discrimination},
  author={Wu, Zhirong and Xiong, Yuanjun and Yu, Stella X and Lin, Dahua},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3733--3742},
  year={2018}
}

@inproceedings{caron2018deep,
  title={Deep clustering for unsupervised learning of visual features},
  author={Caron, Mathilde and Bojanowski, Piotr and Joulin, Armand and Douze, Matthijs},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={132--149},
  year={2018}
}

@article{gidaris2018unsupervised,
  title={Unsupervised representation learning by predicting image rotations},
  author={Gidaris, Spyros and Singh, Praveer and Komodakis, Nikos},
  journal={arXiv preprint arXiv:1803.07728},
  year={2018}
}

@inproceedings{iscen2018mining,
  title={Mining on manifolds: Metric learning without labels},
  author={Iscen, Ahmet and Tolias, Giorgos and Avrithis, Yannis and Chum, Ond{\v{r}}ej},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={7642--7651},
  year={2018}
}

@inproceedings{ye2019unsupervised ,
  title={Unsupervised Embedding Learning via Invariant and Spreading Instance Feature},
  author={Ye, Mang and Zhang, Xu and Yuen, Pong C and Chang, Shih-Fu},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={6210--6219},
  year={2019}
}

@article{cao2019unsupervised,
  title={Unsupervised Deep Metric Learning via Auxiliary Rotation Loss},
  author={Cao, Xuefei and Chen, Bor-Chun and Lim, Ser-Nam},
  journal={arXiv preprint arXiv:1911.07072},
  year={2019}
}




@inproceedings{wang2017deep,
  title={Deep metric learning with angular loss},
  author={Wang, Jian and Zhou, Feng and Wen, Shilei and Liu, Xiao and Lin, Yuanqing},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={2593--2601},
  year={2017}
}


@inproceedings{wang2019multi,
  title={Multi-similarity loss with general pair weighting for deep metric learning},
  author={Wang, Xun and Han, Xintong and Huang, Weilin and Dong, Dengke and Scott, Matthew R},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={5022--5030},
  year={2019}
}

@inproceedings{szegedy2015going,
  title={Going deeper with convolutions},
  author={Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1--9},
  year={2015}
}

@inproceedings{movshovitz2017no,
  title={No fuss distance metric learning using proxies},
  author={Movshovitz-Attias, Yair and Toshev, Alexander and Leung, Thomas K and Ioffe, Sergey and Singh, Saurabh},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={360--368},
  year={2017}
}


@inproceedings{suh2019stochastic,
  title={Stochastic class-based hard example mining for deep metric learning},
  author={Suh, Yumin and Han, Bohyung and Kim, Wonsik and Lee, Kyoung Mu},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={7251--7259},
  year={2019}
}

@inproceedings{ge2018deep,
  title={Deep metric learning with hierarchical triplet loss},
  author={Ge, Weifeng},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={269--285},
  year={2018}
}


@inproceedings{sanakoyeu2019divide,
  title={Divide and conquer the embedding space for metric learning},
  author={Sanakoyeu, Artsiom and Tschernezki, Vadim and Buchler, Uta and Ommer, Bjorn},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={471--480},
  year={2019}
}


@inproceedings{suh2019stochastic,
  title={Stochastic class-based hard example mining for deep metric learning},
  author={Suh, Yumin and Han, Bohyung and Kim, Wonsik and Lee, Kyoung Mu},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={7251--7259},
  year={2019}
}


@inproceedings{oh2016deep,
  title={Deep metric learning via lifted structured feature embedding},
  author={Oh Song, Hyun and Xiang, Yu and Jegelka, Stefanie and Savarese, Silvio},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={4004--4012},
  year={2016}
}


@inproceedings{sohn2016improved,
  title={Improved deep metric learning with multi-class n-pair loss objective},
  author={Sohn, Kihyuk},
  booktitle={Advances in neural information processing systems},
  pages={1857--1865},
  year={2016}
}


@inproceedings{ustinova2016learning,
  title={Learning deep embeddings with histogram loss},
  author={Ustinova, Evgeniya and Lempitsky, Victor},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4170--4178},
  year={2016}
}




@inproceedings{wohlhart2015learning,
  title={Learning descriptors for object recognition and 3d pose estimation},
  author={Wohlhart, Paul and Lepetit, Vincent},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={3109--3118},
  year={2015}
}


@inproceedings{he2018triplet,
  title={Triplet-center loss for multi-view 3d object retrieval},
  author={He, Xinwei and Zhou, Yang and Zhou, Zhichao and Bai, Song and Bai, Xiang},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1945--1954},
  year={2018}
}


@inproceedings{grabner20183d,
  title={3d pose estimation and 3d model retrieval for objects in the wild},
  author={Grabner, Alexander and Roth, Peter M and Lepetit, Vincent},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3022--3031},
  year={2018}
}


@inproceedings{wen2016discriminative,
  title={A discriminative feature learning approach for deep face recognition},
  author={Wen, Yandong and Zhang, Kaipeng and Li, Zhifeng and Qiao, Yu},
  booktitle={European conference on computer vision},
  pages={499--515},
  year={2016},
  organization={Springer}
}



@inproceedings{zhang2016zero,
  title={Zero-shot learning via joint latent similarity embedding},
  author={Zhang, Ziming and Saligrama, Venkatesh},
  booktitle={proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={6034--6042},
  year={2016}
}


@inproceedings{bucher2016improving,
  title={Improving semantic embedding consistency by metric learning for zero-shot classiffication},
  author={Bucher, Maxime and Herbin, St{\'e}phane and Jurie, Fr{\'e}d{\'e}ric},
  booktitle={European Conference on Computer Vision},
  pages={730--746},
  year={2016},
  organization={Springer}
}


@inproceedings{yelamarthi2018zero,
  title={A zero-shot framework for sketch based image retrieval},
  author={Yelamarthi, Sasi Kiran and Reddy, Shiva Krishna and Mishra, Ashish and Mittal, Anurag},
  booktitle={European Conference on Computer Vision},
  pages={316--333},
  year={2018},
  organization={Springer}
}

@inproceedings{tao2016siamese,
  title={Siamese instance search for tracking},
  author={Tao, Ran and Gavves, Efstratios and Smeulders, Arnold WM},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1420--1429},
  year={2016}
}


@inproceedings{yu2018hard,
  title={Hard-aware point-to-set deep metric for person re-identification},
  author={Yu, Rui and Dou, Zhiyong and Bai, Song and Zhang, Zhaoxiang and Xu, Yongchao and Bai, Xiang},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={188--204},
  year={2018}
}


@article{hermans2017defense,
  title={In defense of the triplet loss for person re-identification},
  author={Hermans, Alexander and Beyer, Lucas and Leibe, Bastian},
  journal={arXiv preprint arXiv:1703.07737},
  year={2017}
}


@inproceedings{hadsell2006dimensionality,
  title={Dimensionality reduction by learning an invariant mapping},
  author={Hadsell, Raia and Chopra, Sumit and LeCun, Yann},
  booktitle={2006 IEEE Computer Society Conference on Computer Vision and Pattern Recognition (CVPR'06)},
  volume={2},
  pages={1735--1742},
  year={2006},
  organization={IEEE}
}

@inproceedings{schroff2015facenet,
  title={Facenet: A unified embedding for face recognition and clustering},
  author={Schroff, Florian and Kalenichenko, Dmitry and Philbin, James},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={815--823},
  year={2015}
}



@article{russakovsky2015imagenet,
  title={Imagenet large scale visual recognition challenge},
  author={Russakovsky, Olga and Deng, Jia and Su, Hao and Krause, Jonathan and Satheesh, Sanjeev and Ma, Sean and Huang, Zhiheng and Karpathy, Andrej and Khosla, Aditya and Bernstein, Michael and others},
  journal={International journal of computer vision},
  volume={115},
  number={3},
  pages={211--252},
  year={2015},
  publisher={Springer}
}



@article{kumar2017smart,
  title={Smart mining for deep metric learning},
  author={Kumar, VB and Harwood, Ben and Carneiro, Gustavo and Reid, Ian and Drummond, Tom},
  journal={arXiv preprint arXiv:1704.01285},
  volume={2},
  year={2017}
}


@inproceedings{wu2017sampling,
  title={Sampling matters in deep embedding learning},
  author={Wu, Chao-Yuan and Manmatha, R and Smola, Alexander J and Krahenbuhl, Philipp},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={2840--2848},
  year={2017}
}


@inproceedings{chopra2005learning,
  title={Learning a similarity metric discriminatively, with application to face verification},
  author={Chopra, Sumit and Hadsell, Raia and LeCun, Yann},
  booktitle={2005 IEEE Computer Society Conference on Computer Vision and Pattern Recognition (CVPR'05)},
  volume={1},
  pages={539--546},
  year={2005},
  organization={IEEE}
}

@article{opitz2018deep,
  title={Deep metric learning with bier: Boosting independent embeddings robustly},
  author={Opitz, Michael and Waltner, Georg and Possegger, Horst and Bischof, Horst},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  year={2018},
  publisher={IEEE}
}

@inproceedings{kim2018attention,
  title={Attention-based ensemble for deep metric learning},
  author={Kim, Wonsik and Goyal, Bhavya and Chawla, Kunal and Lee, Jungmin and Kwon, Keunjoo},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={736--751},
  year={2018}
}


@inproceedings{doersch2015unsupervised,
  title={Unsupervised visual representation learning by context prediction},
  author={Doersch, Carl and Gupta, Abhinav and Efros, Alexei A},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={1422--1430},
  year={2015}
}

@inproceedings{zhang2019aet,
  title={Aet vs. aed: Unsupervised representation learning by auto-encoding transformations rather than data},
  author={Zhang, Liheng and Qi, Guo-Jun and Wang, Liqiang and Luo, Jiebo},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2547--2555},
  year={2019}
}

@article{sun2019unsupervised,
  title={Unsupervised Domain Adaptation through Self-Supervision},
  author={Sun, Yu and Tzeng, Eric and Darrell, Trevor and Efros, Alexei A},
  journal={arXiv preprint arXiv:1909.11825},
  year={2019}
}


@inproceedings{mnih2014recurrent,
  title={Recurrent models of visual attention},
  author={Mnih, Volodymyr and Heess, Nicolas and Graves, Alex and others},
  booktitle={Advances in neural information processing systems},
  pages={2204--2212},
  year={2014}
}

@article{ba2014multiple,
  title={Multiple object recognition with visual attention},
  author={Ba, Jimmy and Mnih, Volodymyr and Kavukcuoglu, Koray},
  journal={arXiv preprint arXiv:1412.7755},
  year={2014}
}


@inproceedings{jaderberg2015spatial,
  title={Spatial transformer networks},
  author={Jaderberg, Max and Simonyan, Karen and Zisserman, Andrew and others},
  booktitle={Advances in neural information processing systems},
  pages={2017--2025},
  year={2015}
}

@inproceedings{woo2018cbam,
  title={Cbam: Convolutional block attention module},
  author={Woo, Sanghyun and Park, Jongchan and Lee, Joon-Young and So Kweon, In},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={3--19},
  year={2018}
}


@inproceedings{fu2017look,
  title={Look closer to see better: Recurrent attention convolutional neural network for fine-grained image recognition},
  author={Fu, Jianlong and Zheng, Heliang and Mei, Tao},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={4438--4446},
  year={2017}
}


@inproceedings{chen2019hybrid,
  title={Hybrid-attention based decoupled metric learning for zero-shot image retrieval},
  author={Chen, Binghui and Deng, Weihong},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2750--2759},
  year={2019}
}


@article{wang2019cross,
  title={Cross-Batch Memory for Embedding Learning},
  author={Wang, Xun and Zhang, Haozhi and Huang, Weilin and Scott, Matthew R},
  journal={arXiv preprint arXiv:1912.06798},
  year={2019}
}


@book{manning2008introduction,
  title={Introduction to information retrieval},
  author={Manning, Christopher D and Raghavan, Prabhakar and Sch{\"u}tze, Hinrich},
  year={2008},
  publisher={Cambridge university press}
}


@inproceedings{noroozi2016unsupervised,
  title={Unsupervised learning of visual representations by solving jigsaw puzzles},
  author={Noroozi, Mehdi and Favaro, Paolo},
  booktitle={European Conference on Computer Vision},
  pages={69--84},
  year={2016},
  organization={Springer}
}


@article{he2019momentum,
  title={Momentum contrast for unsupervised visual representation learning},
  author={He, Kaiming and Fan, Haoqi and Wu, Yuxin and Xie, Saining and Girshick, Ross},
  journal={arXiv preprint arXiv:1911.05722},
  year={2019}
}


@article{devries2017improved,
  title={Improved regularization of convolutional neural networks with cutout},
  author={DeVries, Terrance and Taylor, Graham W},
  journal={arXiv preprint arXiv:1708.04552},
  year={2017}
}


@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}


@article{van2014accelerating,
  title={Accelerating t-SNE using tree-based algorithms},
  author={Van Der Maaten, Laurens},
  journal={The Journal of Machine Learning Research},
  volume={15},
  number={1},
  pages={3221--3245},
  year={2014},
  publisher={JMLR. org}
}


@article{ioffe2015batch,
  title={Batch normalization: Accelerating deep network training by reducing internal covariate shift},
  author={Ioffe, Sergey and Szegedy, Christian},
  journal={arXiv preprint arXiv:1502.03167},
  year={2015}
}

@techreport{zhu2002learning,
  title={Learning from labeled and unlabeled data with label propagation},
  author={Zhu, Xiaojin and Ghahramani, Zoubin},
  year={2002},
  institution={Citeseer}
}


@techreport{zhu2005semi,
  title={Semi-supervised learning literature survey},
  author={Zhu, Xiaojin Jerry},
  year={2005},
  institution={University of Wisconsin-Madison Department of Computer Sciences}
}


@article{morel2009asift,
  title={ASIFT: A new framework for fully affine invariant image comparison},
  author={Morel, Jean-Michel and Yu, Guoshen},
  journal={SIAM journal on imaging sciences},
  volume={2},
  number={2},
  pages={438--469},
  year={2009},
  publisher={SIAM}
}

@article{wah2011caltech,
  title={The caltech-ucsd birds-200-2011 dataset},
  author={Wah, Catherine and Branson, Steve and Welinder, Peter and Perona, Pietro and Belongie, Serge},
  year={2011},
  publisher={California Institute of Technology}
}

@inproceedings{KrauseStarkDengFei-Fei_3DRR2013,
  title = {3D Object Representations for Fine-Grained Categorization},
  booktitle = {4th International IEEE Workshop on  3D Representation and Recognition (3dRR-13)},
  year = {2013},
  address = {Sydney, Australia},
  author = {Jonathan Krause and Michael Stark and Jia Deng and Li Fei-Fei}
}



@book{gazzaniga2009cognitive,
  title={The cognitive neurosciences},
  author={Gazzaniga, Michael S},
  year={2009},
  publisher={MIT Press}
}


